Preferences Single-Peaked on a Tree: Multiwinner Elections and Structural Results

A preference profile is single-peaked on a tree if the candidate set can be equipped with a tree structure so that the preferences of each voter are decreasing from their top candidate along all paths in the tree. This notion was introduced by Demange (1982), and subsequently Trick (1989) described an efficient algorithm for deciding if a given profile is single-peaked on a tree. We study the complexity of multiwinner elections under several variants of the Chamberlin-Courant rule for preferences single-peaked on trees. We show that the egalitarian version of this problem admits a polynomial-time algorithm. For the utilitarian version, we prove that winner determination remains NP-hard, even for the Borda scoring function; however, a winning committee can be found in polynomial time if either the number of leaves or the number of internal vertices of the underlying tree is bounded by a constant. To benefit from these positive results, we need a procedure that can determine whether a given profile is single-peaked on a tree that has additional desirable properties (such as, e.g., a small number of leaves). To address this challenge, we develop a structural approach that enables us to compactly represent all trees with respect to which a given profile is single-peaked. We show how to use this representation to efficiently find the best tree for a given profile for use with our winner determination algorithms: Given a profile, we can efficiently find a tree with the minimum number of leaves, or a tree with the minimum number of internal vertices among trees on which the profile is single-peaked. We also consider several other optimization criteria for trees: for some we obtain polynomial-time algorithms, while for others we show NP-hardness results.

==> jair_plus_hyperref.tex <==
%from http://tex.stackexchange.com/questions/43279/fixing-jair-style

\makeatletter

\usepackage[implicit=true,unicode=true,
 bookmarks=true,bookmarksnumbered=true,bookmarksopen=true]
 {hyperref}
\hypersetup{
%  pdftitle={my title},
%  pdfauthor={my name},
%  pdfsubject={my subject},
%  pdfkeywords={my keywords},
  %all links are black to preserve the appearance of a printed paper
  colorlinks=true,
  allcolors=black,
  pdfpagelayout=OneColumn,
  pdfnewwindow=true,
}

\usepackage{refstyle}

%we also use the package rawfonts because this this is copied verbatim
%from the JAIR author kit (http://www.jair.org)
\usepackage{jair, theapa, rawfonts}

%load this package unless you have loaded it earlier
\usepackage{ifpdf}

%only the pdflatex driver can handle hyperlinks that break across lines
%(as citations often do) so we define them only when using pdflatex
\ifpdf

%we add hyperref support with the commands \hyper@natanchorstart and \hyper@natanchorend
\def\@lbibitem[#1]#2{\def\BBA{\BBAA}\item[\hyper@natanchorstart{#2}\@biblabel{#1}\hyper@natanchorend]\if@filesw
	{ \def\BBA{\string\BBA}%
		\def\protect##1{\string ##1\space}\immediate
		\write\@auxout{\string\bibcite{#2}{#1}}%
		\def\BBA{\BBAA}}\fi\ignorespaces}

%load this package unless you have loaded it earlier
\usepackage{ifthen}

%new citation commands. Add more as needed, using the existing ones as templates
%hyperref support is added by using the commands \hyper@natlinkstart and \hyper@natlinkend
\newcommand{\mshortcite}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\shortcite{#2}}{\shortcite[#1]{#2}}\hyper@natlinkend}
\newcommand{\mshortciteA}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\shortciteA{#2}}{\shortciteA[#1]{#2}}\hyper@natlinkend}
\newcommand{\mfullciteA}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\fullciteA{#2}}{\fullciteA[#1]{#2}}\hyper@natlinkend}
\newcommand{\mshortciteR}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\shortciteR{#2}}{\shortciteR[#1]{#2}}\hyper@natlinkend}
\newcommand{\mciteyear}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\citeyear{#2}}{\citeyear[#1]{#2}}\hyper@natlinkend}
\newcommand{\mciteyearR}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\citeyearR{#2}}{\citeyearR[#1]{#2}}\hyper@natlinkend}
\newcommand{\mshortciteS}[2][]{\hyper@natlinkstart{#2}\ifthenelse{\equal{#1}{}}{\shortciteS{#2}}{\shortciteS[#1]{#2}}\hyper@natlinkend}
\newcommand{\mshortciteauthor}[1]{\hyper@natlinkstart{#1}\shortciteauthor{#1}\hyper@natlinkend}
\newcommand{\mfullciteauthor}[1]{\hyper@natlinkstart{#1}\fullciteauthor{#1}\hyper@natlinkend}

\else

%default definitions when not using pdflatex
\let\mcite\shortcite
\let\mcitea\shortciteA
\let\mcitear\fullciteA
\let\mciter\shortciteR
\let\mciteyear\citeyear
\let\mciteyearr\citeyearR
\let\mcites\shortciteS
\let\mciteauthor\shortciteauthor
\let\mciteauthorr\fullciteauthor
\let\mcitetable\mciter

\fi

%use this command unless it is already invoked later in the preamble
\makeatother
